A Beamdump Facility at Jefferson Lab

This White Paper is exploring the potential of intense secondary muon, neutrino, and (hypothetical) light dark matter beams produced in interactions of high-intensity electron beams with beam dumps. Light dark matter searches with the approved Beam Dump eXperiment (BDX) are driving the realization of a new underground vault at Jefferson Lab that could be extended to a Beamdump Facility with minimal additional installations. The paper summarizes contributions and discussions from the International Workshop on Secondary Beams at Jefferson Lab (BDX & Beyond). Several possible muon physics applications and neutrino detector technologies for Jefferson Lab are highlighted. The potential of a secondary neutron beam will be addressed in a future edition.

==> abstracts/abstract_Banerjee.tex <==
%The CERN secondary beam lines of the North and the East Area are designed to deliver beams of secondary and tertiary particles as well as attenuated primary protons and ions from the SPS and PS accelerators. 
%With its diverse portfolio, the CERN experimental areas serve over 200 test beams and experiments per year with more than 2000 users. In context of the Physics Beyond Colliders (PBC) initiative, various new ideas have been presented for exploiting the full scientific potential and intensity for fixed target experiments. These include experiments like AMBER, in the QCD sector, with a rich physics programme ranging from proton radius measurements to meson structure studies, as well as experiments addressing BSM physics, like NA64 and SHiP/BDF, requiring high intensity beams. Requests for different species and high intensities of ion beams have also been brought forward by the NA61 and DiCE/NA60++ collaborations. Various developments and upgrades are therefore being studied and planned for the CERN North and East Area beams during and after the Long Shutdown 3 to be able to serve these diverse requests. 
%The presentation will include an overview of the existing beam lines and facilities at the CERN North and East Area, as well as showcase the upcoming plans for consolidation and upgrades to ensure the optimal physics operation and test beam runs for the coming decades. 


==> abstracts/abstract_Bondi-Spreafico_LDM.tex <==


Astrophysical observations and anomalies in processes involving electromagnetic currents, such as the muon anomalous magnetic moment, suggest the possible existence of a new form of matter that does not interact directly with light: Dark Matter (DM). While the gravitational effects of DM are well established, its particle nature remains unknown despite extensive experimental efforts. Traditional searches have largely focused on the WIMP paradigm, which postulates weakly interacting massive particles with masses above 1 GeV, but have so far yielded no conclusive evidence. This has motivated increasing interest in the exploration of Light Dark Matter (LDM) in the MeV–GeV mass range. Such a scenario is theoretically well motivated under the hypothesis of a thermal origin of DM: interactions with Standard Model particles would have enabled thermal equilibrium in the early universe, with the subsequent cosmic expansion freezing the DM abundance at its present value. For sub-GeV thermal DM, this mechanism requires the presence of new light mediators in the dark sector, capable of providing the necessary annihilation channels. Such mediators must couple to visible matter and be neutral under the Standard Model (SM) U(1) gauge group. Theoretical extensions of the Standard Model (SM) that introduce new interactions and particles are highly constrained. Among the minimal and well-motivated scenarios are the vector portal, mediated by a dark photon; the scalar portal, involving mixing with the Higgs boson; and the neutrino portal, mediated by heavy neutral leptons. Vector and scalar portals are particularly relevant in the case of Dark Matter with masses in the MeV–GeV range.
A representative benchmark model is the vector portal mediated by a dark photon ($A'$), kinetically mixed with the SM hypercharge~\cite{Holdom:1985ag}. In this scenario, LDM is produced via real or virtual $A'$ decays. The fundamental parameters of the model are the dark photon and LDM masses ($m_A'$, $m_\chi$), the LDM–dark photon coupling ($g_D \equiv \sqrt{4\pi\alpha_D}$), and the kinetic mixing parameter ($\varepsilon$).

On the experimental side, extensive efforts have been devoted to probing these scenarios. Existing data, often collected in experiments optimized for other physics goals, have been reanalyzed to set exclusion limits in the parameter space of the different models. At the same time, a new generation of dedicated experiments has already started data taking or is planned for the near future, aiming to explore these portals with unprecedented sensitivity. For a comprehensive overview of the theoretical landscape of light dark matter, current experimental constraints, and future prospects, we refer the reader to the FIPs 2022 Workshop Report~\cite{Antel:2023hkf}. Present accelerator technology provides high intensity particle beams of moderate energy that are well suited for the discovery of LDM~\cite{Battaglieri:2017aum, Krnjaic:2022ozp}.  In particular, electron beam dump experiments have been shown to have high sensitivity to light dark matter~\cite{Batell:2014mga, Andreev:2021fzd, Bondi:2017gul}.  In these experiments, light dark matter particles ($\chi {\bar\chi}$ pairs) are conjectured to be produced  when the electron
beam interacts with nucleons and electrons  in the beam dump via $A'$ radiative process ($A'$-\textit{strahlung}) or annihilation (resonant and non-resonant) of positrons produced by the electromagnetic shower generated therein~\cite{Izaguirre:2013uxa, Marsicano:2018glj, Marsicano:2018krp}. A detector located downstream of the beam dump, shielded from SM background particles (other than neutrinos), could be sensitive to the interaction of DM $\chi$s. 
Jefferson Lab, providing one of the most intense and continuous electron beams worldwide, offers unique conditions for exploring the dark sector. The Beam Dump eXperiment (BDX) will be the first full-scale beam-dump experiment explicitly designed for DM searches. Scheduled to operate in parallel with the MOLLER experiment, BDX will exploit CEBAF’s high-current 11 GeV electron beam directed onto the Hall A beam dump. A dedicated detector will be placed about 20 m downstream of the dump, behind substantial shielding (concrete $\sim$5.5m, dirt$\sim$7m, lead$\sim$1.5m and steel$\sim$3.5m) that will eliminate all SM backgrounds except neutrinos.
The detector will consist of a about one-cubic-meter electromagnetic calorimeter, made of BGO and PbWO$_4$ crystals, surrounded by plastic scintillators and lead layers serving as active and passive veto systems. The characteristic signature of $\chi$–electron scattering will be an electromagnetic shower with deposited energy above 10 MeV, efficiently detectable by the calorimeter. Given the small production cross sections and interaction rates, very high statistics are required. With the expected integrated beam exposure (total accumlated charge expected $\sim$10$^{22}$), BDX will achieve sensitivity to previously unexplored regions of parameter space, exceeding the reach of existing and planned experiments by up to two orders of magnitude, as illustrated in Fig.~iXX.



\paragraph{Additional Information}

\begin{description}
    \item[What type of beam is required?] Light dark matter particles. 
    \item[What type of targets and instrumentation are required?] BDX will use total-absorption crystal calorimeters behind several meters of heavy material shielding (steel and lead).
    \item[What type of  infrastructure is required?] BDX facility with a shielding behind the detector made of 1.5m of lead and 3.5m of steel.  
\end{description}




==> abstracts/abstract_Bondi_Spreafico_MuonDS.tex <==
Medium-energy electron beam-dump experiments provide an intense sources of secondary muons.
These particles can be used to search for muon-coupling light dark scalars that may explain the
(g-2)$_{\mu}$ anomaly. The so-called (g-2)$_{\mu}$ has provided a strong motivation for light hidden particles searches, opening a window to new physics
beyond the Standard Model (SM). Popular candidates
such as dark photons and dark Higgs have been tightly
scrutinized as a possible explanation for such anomaly.
However, this hypothesis has been excluded by existing
measurements (see e.g. [,]). Nevertheless, other solutions, such as a new light particle that dominantly couples to muons, remain viable and deserve attention. In
this paper, we examine models with a newIn this work, we focused on the minimal model that could explain the $(g-2)_\mu$ anomaly: a new, \textit{leptophilic} scalar dark matter state (\textit{Dark Scalar} or $S$) that couples only to muons. A detailed description of the theoretical model is reported in Ref.~\cite{Chen:2017awl, Marsicano:2018vin} and references therein. 
In this model, the main process responsible for  $S$ emission by an impinging muon on a fixed target is the so-called “radiative” production $\mu$~+~N$\xrightarrow{}$$\mu$~+~N~+~$S$.
The incident muon interacts with a target nucleus, N, by exchanging a photon, $\gamma$, and radiates the $S$.
 For the mass range  ($m_S<2m_\mu$), $S$ could only decay  into two photons $m_\mu/m_S$ ~\cite{Chen:2017awl}. Different experimental techniques can be used to search for muon-coupling light dark scalars. Among them, medium-energy electron beam dump experiments, providing an intense source of secondary muons, cover a broad area in the $g_\mu$ vs. Different experimental techniques can be used to search for muon-coupling light dark scalars. Among them, medium-energy high-intensity electron beam dump experiments, providing an intense source of secondary muons, cover a broad area in the $g_\mu$ vs.  $m_S$ parameter space. In this work we



\paragraph{Additional Information}

\begin{description}
    \item[What type of beam is required?] Light dark matter particles. 
    \item[What type of targets and instrumentation are required?] BDX will use total-absorption crystal calorimeters behind several meters of heavy material shielding (steel and lead).
    \item[What type of  infrastructure is required?] BDX facility with a shielding behind the detector made of 1.5m of lead and 3.5m of steel.  
\end{description}




==> abstracts/abstract_Liu.tex <==
%\author[a]{Marco Battaglieri,}
%\author[i]{Mariangela Bondi,}
%\author[b]{Ana Botti,}
%\author[b]{Brenda A.~Cervantes-Vergara,}
%\author[a,l]{Raffella De Vita,}
%\author[d]{Rouven Essig,}
%\author[b]{Juan Estrada,}
%\author[e]{Peiran Li,}
%\author[d,f]{Megan McDuffie,}
%\author[g]{Santiago Perez,}
%\author[g]{Dario Rodrigues,}
%\author[h]{Ryan Plestid,}
%\author[a]{Marco Spreafico,}
%\author[b]{Javier Tiffenberg,}
%\author[d,f]{Hailin Xu}
%\author{and the BDX Collaboration}

%\affiliation[a]{Istituto Nazionale di Fisica Nucleare, Sezione di Genova e Dipartimento di Fisica dell’Universit\`a, 16146 Genova, Italy}
%\affiliation[b]{Fermi National Accelerator Laboratory, IL, USA}
%\affiliation[d]{C.N. Yang Institute for Theoretical Physics, Stony Brook University, Stony Brook, NY 11794}
%\affiliation[f]{Physics and Astronomy Department, Stony Brook University, NY 11794, USA}
%\affiliation[g]{Universidad de Buenos Aires, Buenos Aires, Argentina}
%\affiliation[h]{Walter Burke Institute for Theoretical Physics, \\ California Institute of Technology, Pasadena, CA 91125, USA}
%\affiliation[i] {Istituto Nazionale di Fisica Nucleare, Sezione di Catania, 95123 Catania, Italy}
%\affiliation[l]{Thomas Jefferson National Accelerator Facility,  VA 23606, USA}

% \emailAdd{javiert@fnal.gov}
% \emailAdd{rouven.essig@stonybrook.edu}
% \emailAdd{battaglieri@ge.infn.it}

%RE: re-defined abstract in jheppub.sty to call it Executive Summary
Millicharged particles can be produced in high-intensity electron beam dumps and detected with small ultralow-threshold Skipper-Charge-Coupled-Devices (Skipper-CCDs). 
In particular, Skipper-CCDs can be placed behind the beam dump in Hall~A at Jefferson Lab near the planned Beam Dump eXperiment (BDX) detector.  A large flux of millicharged particles can be produced in the dump, allowing even a modest $2\times 14$ array of Skipper-CCDs to exceed the sensitivity of all existing searches for millicharged particle masses below 1.5~GeV, and to be either competitive or world-leading when compared to other proposed experiments. We discuss the scientific motivation for millicharged particles, their production, and their detection, as well as the synergies with the planned BDX experiment. 
This talk correponds to an LOI submitted by the team.
%Augmenting the BDX detector with Skipper-CCDs can extend the physics reach to other dark-sector particles, such as millicharged particles.
%\recomment{To discuss: go over comments; authors; contact people; who/how submit? what is sensitivity to (long-lived) visibly decaying dark photons in BDX detector?}

%\section{Additional Information}
% %
% References to Jefferson Lab's secondary beams~\cite{Battaglieri:2023gvd} as well as the BDX~\cite{BDX:2019afh} and BDX-MINI~\cite{Battaglieri:2022dcy} Experiments are in the sample {\tt references.bib} file. Please use {\sc BibTeX} for references, so that we can compile the White Paper. Figures, tables, and formulas are allowed and encouraged in this extended abstract.

The proposed Beam Dump Experiment (BDX) at Jefferson Lab~\cite{BDX:2014pkr,BDX:2016akw,BDX:2017jub,BDX:2019afh} is uniquely positioned to perform world-leading searches for light dark-sector particles. By delivering $10^{22}$ electrons on target (EOT)—a three-orders-of-magnitude increase over the SLAC-mQ experiment~\cite{Prinz:1998ua}—BDX will dramatically enhance sensitivity to new weakly interacting particles. Furthermore, the main detector of BDX, placed 20~meter downstream of the target, comprises a segmented electromagnetic calorimeter (ECal) made of approximately 3 tons ($\sim$1 m$^3$) of scintillating crystals (BGO and PbWO$_4$). A critical feature of the BDX detector is its dual-layer active veto system, designed to suppress background events. This system consists of inner and outer layers of 1.0 cm-thick plastic scintillator paddles, which detect and veto incoming charged particles such as cosmic rays and beam-related muons. Between the ECal and the veto layers, a 5 cm-thick lead shield is installed to absorb secondary particles and reduce the likelihood of electromagnetic showers depositing energy in the veto counters, thereby enhancing the detector's sensitivity to genuine dark matter interactions. 
To effectively discriminate between potential dark matter signals and background events, the BDX detector employs an energy threshold of hundreds of MeV. This threshold is optimized to minimize contributions from cosmologic and beam-related backgrounds, while maintaining sensitivity to the expected energy deposition from LDM interactions. In summary, the BDX main detector's comprehensive design—featuring a high-intensity electron beam, close detector placement, sensitive calorimeter with dual-layer active veto system, and an optimized energy threshold—enables it to achieve high sensitivity to light dark matter particles while effectively mitigating background noise. 

The conventional electron recoil detector always carries the high-threshold regime $\sim\mathcal{O}(100~\text{MeV})$. However, in certain models the interactions of the dark sector are more pronounced in low-energy scattering events. Especially, for dark matter with $m<\mathcal{O}(10~\text{MeV})$, a threshold of $\sim$100~MeV will cut out a huge fraction of signal events. In this letter, we follow~\cite{Essig:2024dpa} and \textbf{advocate for augmenting the BDX detector with ultralow-threshold sensors: Skipper-Charge Coupled Devices (Skipper-CCDs)}~\cite{Tiffenberg:2017aac}. This is motivated by the fact that some dark sector particle candidates that scatter in a detector medium prefer to transfer very little energy to it. It not only complements the high energy threshold of the main detector, but can also be positioned behind it, making full use of the existing shielding and veto system.  Moreover, the SENSEI collaboration performed an opportunistic search for mCPs using their Skipper-CCD detector, which happened to be located downstream of the NuMI beam in the MINOS cavern at Fermilab~\cite{SENSEI:2023gie}.  Despite the fact that only a single 2-gram Skipper-CCD was in operation and the SENSEI detector was $\sim$1~km away from the target, world-leading limits were placed on mCPs detection, since the low energy threshold of the Skipper-CCD can enhance the sensitivity to dark-sector particles compared to a typical detector that has a much higher threshold. 
The Oscura collaboration has proposed using a 1-kg Skipper-CCD detector to search for mCPs using the NuMI beam as part of an engineering test on the way to developing a 10-kg dark matter detector~\cite{Oscura:2023qch}. 
Skipper-CCDs have also been used in mCP searches produced in reactors~\cite{CONNIE:2024off}.

A significant advantage of low-threshold detectors is that they are small and versatile, and relatively easy to deploy. Integrating Skipper-CCD technology into BDX will enable an unprecedented sensitivity to a broad range of light dark-sector scenarios—including millicharged particles, dark photons, and other feebly interacting particles—providing an unparalleled opportunity to explore physics beyond the Standard Model.

%\section{Tracks}
%(3) dark matter and dark sector searches

%\section{Application to Jefferson Lab's Secondary Beams}

\begin{description}
    \item[What type of beam is required?] 
    
    Consider particle type, beam purity, fluxes, energy, and other distributions. 
    Electron beam. No separate beam time required. It runs concurrently with the existing program.
    The small size, low power requirements, and passive operational mode of the Skipper-CCD detector ensure it can run continuously without interfering with the primary goals of the Moller program. Its operation will be synchronized with the beam structure for background rejection and will not place significant additional demands on beam time, support staff, or infrastructure.
    \item[What type of targets and instrumentation are required?]  
    
    A Skipper-CCD detector.  
    
    \item[What type of  infrastructure is required?] 
    
    See the table.


\end{description}

\begin{table}[t]
\centering
\caption{Estimated power consumption of supporting systems for the Skipper-CCD detector.}
\begin{tabular}{l c c}
\hline
\textbf{Subsystem} & \textbf{Component} & \textbf{Power Consumption} \\
\hline
Vacuum System & Turbo pump + backing pump & 100–300 W \\
Cryogenic Cooling & Cryocooler  & 300–600 W \\
Readout Electronics & Controller + digitizers & 50–150 W \\
Computing & Control + local storage & 200-300 W \\
\hline
\end{tabular}
\label{tab:power}
\end{table}


==> abstracts/abstract_Tena_Vidal.tex <==
The next generation of neutrino experiments aims to address some of the most fundamental questions in particle physics, including the search for charge-parity (CP) violation in the lepton sector, tests of the three-flavor oscillation paradigm, and the study of supernova explosions. Achieving these goals requires an unprecedented understanding of neutrino--nucleus interactions across a wide energy range, from MeV to TeV. However, modeling neutrino interactions is particularly challenging due to the non-perturbative nature of QCD in the relevant energy regimes and nuclear physics. As a result, models depend heavily on experimental input. 
%In this talk, we describe how electron-scattering data from Jefferson Lab experiments including 
The beamdump facility could be used to constrain neutrino event generators, ultimately reducing systematic uncertainties in upcoming neutrino measurements. 


==> abstracts/abstract_Wood.tex <==
Primarily undergraduate institutions (PUIs) play a critical role in advancing scientific education and research by fostering hands-on learning and mentorship opportunities for students. 
%The National Science Foundation (NSF) Major Research Instrumentation (MRI) grants provide PUIs with access to state-of-the-art equipment, enabling cutting-edge research that would otherwise be financially unattainable. These grants enhance undergraduate training by preparing students for graduate studies and STEM careers. Faculty at PUIs benefit from MRI grants through increased research productivity and opportunities to collaborate with larger institutions. By funding specialized instrumentation, NSF MRI grants elevate the quality of research at PUIs, and in the case of a Beam Dump Facility, increase the involvement of a PUI at Jefferson Lab. 
%In this article, I will discuss my experience as a professor and researcher at a PUI and will share my vision of a collaborative NSF MRI with other PUI and R1 institutions.
%
%The Beam Dump Experiment (BDX) at the Thomas Jefferson National Accelerator Facility (Jefferson Lab) represents a frontier in the search for dark matter, leveraging the lab’s high-intensity electron beam to probe light dark matter particles produced in electron-nucleus interactions \citep{battaglieri2017cosmicvisionsnewideas}. Located behind the beam dump in Hall A, BDX facility will utilize a compact detector to capture potential dark matter candidates that interact weakly with standard matter. The experimental design exploits the high-luminosity Continuous Electron Beam Accelerator Facility (CEBAF) to produce secondary particles, such as muons and neutrinos, offering a unique opportunity to explore beyond-Standard-Model physics. Future experimental areas at Jefferson Lab, particularly those dedicated to secondary beams, are poised to expand this research. 
%
PUIs %like Canisius University 
can play a pivotal role for the beamdump facility through participation in National Science Foundation (NSF) Major Research Instrumentation (MRI) grants. By focusing on the development and testing of detector components or developing software, PUIs can contribute meaningfully to large-scale experiments while providing transformative research opportunities for undergraduates. 

%\paragraph{Role of PUIs in Detector Development}
%Canisius University, a Jesuit institution in Buffalo, New York, with a strong emphasis on undergraduate education, is well-positioned to contribute to the BDX facility through detector and software development. The university has a history of engaging students in hands-on research, making it an ideal candidate for NSF MRI funding to acquire advanced instrumentation. Specifically, Canisius can focus on developing and testing critical detector components, such as plastic scintillators and SiPMs, which are integral to the BDX’s ability to detect rare particle interactions. 

Through an NSF MRI grant, PUIs could acquire equipment like precision oscilloscopes, light-tight testing chambers, and cosmic ray test stands to characterize scintillator and SiPM performance. Undergraduates would lead efforts to optimize scintillator light yield, measure SiPM gain, and assess detector response to cosmic muons, providing data critical to the design phase. These activities not only advance the experiment but also immerse students in authentic research, aligning with the NSF’s goal of broadening participation in STEM \citep{NSF2022}. By integrating these efforts into the curriculum, a PUI can offer course-based undergraduate research experiences, ensuring that a diverse student body gains exposure to particle physics.

%\paragraph{Collaboration with Research Institutions}
The success of PUI’s involvement hinges on collaboration with other PUIs and established research institutions. An NSF MRI grant can facilitate a consortium approach, where multiple institutions pool resources to support the BDX. These institutions can share instrumentation and expertise, with each focusing on complementary aspects of detector development. 
%
A partnership with Jefferson Lab will further impact a PUI. Jefferson Lab will expose the students to the experimental infrastructure that a PUI can not afford. Faculty and students would participate in joint workshops, detector assembly, and commissioning at Jefferson Lab, gaining access to a world-class facility. These collaborations ensure that PUI contributions meet rigorous scientific standards while fostering mentorship networks that support undergraduate researchers.
%
%\paragraph{Impact and Broader Implications}
The involvement of an PUI in an NSF MRI grant for the BDX has far-reaching implications. %Scientifically, PUI contributions to detector development enhance the experiment’s sensitivity, potentially leading to breakthroughs in dark matter detection. 
Educationally, undergraduates gain hands-on experience with cutting-edge instrumentation, preparing them for graduate studies or careers in STEM. This is particularly impactful for undergraduate students who may lack access to research resources at larger institutions.
%
Economically, the grant would make a tremendous impact on a PUI.  %A few \$100,000 would go a long way in supporting an undergraduate research group.  
These funds would support summer stipends for both faculty and students, travel to Jefferson Lab and conferences, and purchase state-of-the-art equipment.  Most research groups at PUIs operate on a shoestring budget.  A NSF MRI would allow for more students to join cutting-edge research and bring valuable resources to a PUI.  There is a growing demand for skilled researchers, and with the proper support, PUIs like Canisius University can paly a vital role.

%\paragraph{Conclusion}
% Summarizing the potential of PUI involvement
%The participation of PUIs in an NSF MRI grant to support the Beam Dump Experiment at Jefferson Lab exemplifies how PUIs can contribute to frontier physics research. By focusing on detector and software development, collaborating with other institutions, and engaging undergraduates in meaningful research, Canisius can enhance the BDX’s scientific output while advancing educational and workforce goals. This model of PUI involvement not only strengthens experiments like the BDX but also ensures that the next generation of physicists is educated, skilled, and prepared to tackle the universe’s greatest mysteries.

